Structure-Aware Language Model Pretraining Improves Dense Retrieval on Structured Data

This paper presents Structure Aware Dense Retrieval (SANTA) model, which encodes user queries and structured data in one universal embedding space for retrieving structured data. SANTA proposes two pretraining methods to make language models structure-aware and learn effective representations for structured data: 1) Structured Data Alignment, which utilizes the natural alignment relations between structured data and unstructured data for structure-aware pretraining. It contrastively trains language models to represent multi-modal text data and teaches models to distinguish matched structured data for unstructured texts. 2) Masked Entity Prediction, which designs an entity-oriented mask strategy and asks language models to fill in the masked entities. Our experiments show that SANTA achieves state-of-the-art on code search and product search and conducts convincing results in the zero-shot setting. SANTA learns tailored representations for multi-modal text data by aligning structured and unstructured data pairs and capturing structural semantics by masking and predicting entities in the structured data. All codes are available at https://github.com/OpenMatch/OpenMatch.

==> figure/csn_attention.tex <==
\begin{figure*}[t]
\centering
\includegraphics[scale=0.38]{image/csn_attention.png}
\caption{Visualization of Attention Distribution of SANTA on Different Type Code. The cross attention weight distributions from the decoder module to encoded token embeddings are plotted. Darker blue indicates a higher attention weight.}
\label{fig:csn attention}
\end{figure*}

==> table/Antinoise.tex <==
\begin{table}
\begin{center}
\small
\resizebox{0.40\textwidth}{!}{
\begin{tabular}{l| r r}
\hline
{\textbf{Model}} & {\textbf{T5(w/ SDA)}} & {\textbf{T5(w/ SDA-raw)}} \\ 
\hline
Code & 45.0 & 37.8  \\
Code (w/ mask) & 31.7 & 20.2  \\
Difference & 13.3 & 17.6  \\

\hline
\end{tabular}}
\caption{Comparison of The Noise Immunity of SDA and SDA-raw. Code refers to the original test set, code (w/ mask) refers to the test set with added noise.}
\label{tab:antinoise}
\end{center}
\end{table}

==> table/antinoisecase.tex <==
\begin{table*}[!ht]
\small
\begin{tabular}{p{0.1\linewidth}|p{0.4\linewidth}|p{0.4\linewidth}}
\hline 
\textbf{Model}  & {\textbf{T5(w/ SDA)}} & {\textbf{T5(w/ SDA-raw)}} 
\tabularnewline 
\hline
\textbf{Query} & \multicolumn{2}{p{0.8\linewidth}}{Returns True if credentials expire sooner than specified.}
\tabularnewline 
\hline
top5 code 
&
1.Returns True if credentials expire sooner than specified. 2.True if credentials are valid False if expired. 3.Check if token expires or not. 4.Determine if the confirmation has expired. 5.Checks to see if a cache file needs to be refreshed. &
1.Returns True if credentials expire sooner than specified. 2.Returns True if there are valid credentials for the current user. 3.True if credentials are valid False if expired. 4.Check if token expires or not. 5.Handles the message shown when we are ratelimited.
\tabularnewline 
\hline
top5 code with masked entities 
&
1.Return a canonical tautomer by enumerating and scoring all possible tautomers. 2.Returns True if credentials expire sooner than specified. 3.Run tasks in a greenlet pulling from the workers task queue. 4.Check if the specifed file exists and is not empty. 5.Call this at Python startup to perhaps measure coverage.
&
1.Plotting wrapper for pitch contours. 2.Check if the specifed file exists and is not empty. 3.Get or create a user class of the given type. 4.Build command line argument parser. 5.Store the union of sets src args into a new set named dest. Returns the number of keys in the new set.
\tabularnewline 
\hline 

\end{tabular}
  \caption{Case of Noise Immunity. For the given query example, we use T5 (w/SDA) and T5 (w/SDA-raw) to retrieve on the original test set and the test set with masked entities, respectively, and collect the corresponding descriptions of the retrieved top5 code.}
  \label{tab:antinoisecase}
\end{table*}

==> table/maskstrategy.tex <==
\begin{table}
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l | c  c}
\hline
\textbf{Model} & \textbf{Code Search} & \textbf{Product Search}\\ \cline{2-3}
& MRR & NDCG \\
\hline
 SANTA (Random Mask) & 42.11 & 80.99 \\
 SANTA (Entity Mask) & 47.28 & 81.41 \\
\hline
\end{tabular}}
\caption{The impact of different mask strategies on Structured data retrieval. Random Mask employ the same 15\% mask rate as T5 and ensure the average span length to be 2. Entity Mask is mask all entities in structure data.}
\label{tab:maskstrategy}
\end{table}
